Performance Portable Solid Mechanics via Matrix-Free $p$-Multigrid

Finite element analysis of solid mechanics is a foundational tool of modern engineering, with low-order finite element methods and assembled sparse matrices representing the industry standard for implicit analysis. We use performance models and numerical experiments to demonstrate that high-order methods greatly reduce the costs to reach engineering tolerances while enabling effective use of GPUs; these data structures also offer up to 2x benefit for linear elements. We demonstrate the reliability, efficiency, and scalability of matrix-free $p$-multigrid methods with algebraic multigrid coarse solvers through large deformation hyperelastic simulations of multiscale structures. We investigate accuracy, cost, and execution time on multi-node CPU and GPU systems for moderate to large models (millions to billions of degrees of freedom) using AMD MI250X (OLCF Crusher), NVIDIA A100 (NERSC Perlmutter), and V100 (LLNL Lassen and OLCF Summit), resulting in order of magnitude efficiency improvements over a broad range of model properties and scales. We discuss efficient matrix-free representation of Jacobians and demonstrate how automatic differentiation enables rapid development of nonlinear material models without impacting debuggability and workflows targeting GPUs. The methods are broadly applicable and amenable to common workflows, presented here via open source libraries that encapsulate all GPU-specific aspects and are accessible to both new and legacy code, allowing application code to be GPU-oblivious without compromising end-to-end performance on GPUs.

==> audience.tex <==
%!TEX root = SC22_draft_stengel_v0.tex

\section*{Extra info for class - not part of draft}

\subsection*{Audience}
Attendees and readers of the Super Computing 2022 conference. We are submitting to the applications track so it will be catered towards people who model various solid (and fluid) mechanics problems, people who are interested in efficient solvers, as well as those interested in high performance computing (HPC) capable software.

Goal: sell to readers that $p$-multigrid for AMG as a useful method for solving solid mechanics simulations. Do this by investigating the performance vs accuracy trade offs of benchmark problems. 

\subsection*{Expected background knowledge}

\begin{itemize}
	\item portable - can be run on different computers running different operating systems with little to no modification.
	\item scalable - minimal performance loss to communication between nodes. i.e. runs large simulations efficiently in parallel
	\item preconditioner - conditions a given problem into a form that is more suitable for numerical solving methods
	\item Strong scaling - how the solution time varies with the number of processors for a fixed {\it total} problem size.
	\item Weak scaling - how the solution time varies with the number of processors for a fixed problem size {\it per processor}.
	\item L2 error $= \sum\limits_{i=1}^N (y_{true} - y_{predicted})^2$. $y_{true}$ in this case is the expected solution, usually found with Method of Manufacutred Solutions (assume/manufacture a solution to compare your solver to).
\end{itemize}

